Towards bridging the gap: Systematic sim-to-real transfer for diverse legged robots

Legged robots must achieve both robust locomotion and energy efficiency to be practical in real-world environments. Yet controllers trained in simulation often fail to transfer reliably, and most existing approaches neglect actuator-specific energy losses or depend on complex, hand-tuned reward formulations. We propose a framework that integrates sim-to-real reinforcement learning with a physics-grounded energy model for permanent magnet synchronous motors. The framework requires a minimal parameter set to capture the simulation-to-reality gap and employs a compact four-term reward with a first-principle-based energetic loss formulation that balances electrical and mechanical dissipation. We evaluate and validate the approach through a bottom-up dynamic parameter identification study, spanning actuators, full-robot in-air trajectories and on-ground locomotion. The framework is tested on three primary platforms and deployed on ten additional robots, demonstrating reliable policy transfer without randomization of dynamic parameters. Our method improves energetic efficiency over state-of-the-art methods, achieving a 32 percent reduction in the full Cost of Transport of ANYmal (value 1.27). All code, models, and datasets are publicly available.

==> acronyms.tex <==
\DeclareAcronym{ai}{
  short = AI ,
  long  = Artificial Intelligence
}
\DeclareAcronym{ml}{
  short = ML ,
  long  = Machine Learning
}
\DeclareAcronym{rl}{
  short = RL ,
  long  = Reinforcement Learning
}
\DeclareAcronym{pdd}{
  short = PDD ,
  long  = Pseudo-Direct Drive
}
\DeclareAcronym{cmaes}{
  short = CMA-ES ,
  long  = Covariance Matrix Adaptation Evolution Strategy
}
\DeclareAcronym{bo}{
  short = BO ,
  long  = Bayesian Optimization
}
\DeclareAcronym{ppo}{
  short = PPO ,
  long  = Proximal Policy Optimization
}
\DeclareAcronym{pmsm}{
  short = PMSM ,
  long  = Permanent Magnet Synchronous Motor
}
\DeclareAcronym{bldc}{
  short = BLDC ,
  long  = Brushless Direct Current Motor
}
\DeclareAcronym{foc}{
  short = FOC ,
  long  = Field-Oriented Control
}
\DeclareAcronym{pace}{
  short = PACE ,
  long  = Precise Adaptation through Continuous Evolution
}
\DeclareAcronym{ftd}{
  short = FTD ,
  long  = Foot-Touchdown
}
\DeclareAcronym{cot}{
  short = CoT ,
  long  = Cost of Transport
}
\DeclareAcronym{cod}{
  short = CoD ,
  long  = Cost of Drives
}
\DeclareAcronym{coe}{
  short = CoE ,
  long  = Cost of Electronics
}
\DeclareAcronym{col}{
  short = CoL ,
  long  = Cost of Locomotion
}
\DeclareAcronym{soc}{
  short = SoC ,
  long  = State of Charge
}
\DeclareAcronym{fft}{
  short = FFT ,
  long  = Fast Fourier Transform
}
